A Deep Search For Faint Galaxies Associated With Very Low-redshift C IV Absorbers: II. Program Design, Absorption-line Measurements, and Absorber Statistics

To investigate the evolution of metal-enriched gas over recent cosmic epochs as well as to characterize the diffuse, ionized, metal-enriched circumgalactic medium (CGM), we have conducted a blind survey for C IV absorption systems in 89 QSO sightlines observed with the Hubble Space Telescope (HST) Cosmic Origins Spectrograph (COS). We have identified 42 absorbers at z < 0.16, comprising the largest uniform blind sample size to date in this redshift range. Our measurements indicate an increasing C IV absorber number density per comoving path length (dN/dX = 7.5 +/- 1.1) and modestly increasing mass density relative to the critical density of the Universe (Omega(C IV) = 10.0 +/- 1.5 x 10^-8 ) from z ~ 1.5 to the present epoch, consistent with predictions from cosmological hydrodynamical simulations. Furthermore, the data support a functional form for the column density distribution function that deviates from a single power-law, also consistent with independent theoretical predictions. As the data also probe heavy element ions in addition to C IV at the same redshifts, we identify, measure, and search for correlations between column densities of these species where components appear aligned in velocity. Among these ion-ion correlations, we find evidence for tight correlations between C II and Si II, C II and Si III, and C IV and Si IV, suggesting that these pairs of species arise in similar ionization conditions. However, the evidence for correlations decreases as the difference in ionization potential increases. Finally, when controlling for observational bias, we find only marginal evidence for a correlation (86.8% likelihood) between the Doppler line width b(C IV) and column density N(C IV).

==> CorrStats.tex <==
\begin{table*}[!t] 
\caption{Correlation Statistics of Ion Column Densities} 
\begin{center} 
\begin{threeparttable} 
\begin{tabular}{ccccccccc} 
\toprule 
Ion 1 & Ion 2  & $\tau_{ss}$\tnote{a}  & $P_{\tau ss}$\tnote{b}  & $\tau_{sd} $\tnote{c} & P$_{\tau sd}$\tnote{d} & $\Phi_{I}(1)$ (eV)\tnote{e} & $\Phi_{I}(2)$ (eV)\tnote{f} & $|\Delta \Phi|$ (eV) \\ 
\hline 
C IV & C II & 0.4286 & 0.0559 & 0.3744 & 0.1314 & 47.8 & 11.3 & 36.5 \\ 
C IV & O I & 0.0585 & 0.7698 & 0.0 & 1.0 & 47.8 & 0.0 & 47.8 \\ 
C IV & Si III & 0.4729 & 0.0242 & 0.3744 & 0.1353 & 47.8 & 16.3 & 31.5 \\ 
C IV & Si IV & 0.5867 & 0.0091 & 0.4933 & 0.0483 & 47.8 & 33.5 & 14.3 \\ 
C IV & O VI & 1.1667 & 0.0154 & 1.2778 & 0.0159 & 47.8 & 113.9 & 66.1 \\ 
C IV & N V & 0.3922 & 0.0244 & 0.4052 & 0.0224 & 47.8 & 77.5 & 29.7 \\ 
C II & Si III & 1.0292 & 0.0014 & 1.076 & 0.0009 & 11.3 & 16.3 & 5.0 \\ 
C II & Si IV & 0.8182 & 0.0172 & 0.8182 & 0.0172 & 11.3 & 33.5 & 22.2 \\ 
Si II & Si IV & 0.2821 & 0.4017 & 0.2821 & 0.4017 & 8.1 & 33.5 & 25.4 \\ 
Si III & Si IV & 0.8382 & 0.0057 & 0.8971 & 0.0034 & 16.3 & 33.5 & 17.2 \\ 
C II & Si II & 1.1048 & 0.0041 & 1.1048 & 0.0041 & 11.3 & 8.1 & 3.2 \\ 
Si II & Si III & 0.8235 & 0.014 & 0.8235 & 0.0145 & 8.1 & 16.3 & 8.2 \\ 
C IV & Si II & 0.2333 & 0.2427 & 0.1267 & 0.5993 & 47.8 & 8.1 & 39.7 \\ 
\hline 
\end{tabular} 
\begin{tablenotes} 
\item[a] {\scriptsize The Kendall tau correlation coefficient between the column densities of Ion 1 and Ion 2, assuming that lines flagged as saturated yield lower limits for their column densities.} 
\item[b] {\scriptsize Probablility that a correlation does not exist between the column densities of Ion 1 and Ion 2, assuming that lines flagged as saturated yield lower limits for their column densities.} 
\item[c] {\scriptsize The Kendall tau correlation coefficient between the column densities of Ion 1 and Ion 2, assuming that lines flagged as saturated yield reliable column densities.} 
\item[d] {\scriptsize Probablility that a correlation does not exist between the column densities of Ion 1 and Ion 2, assuming that lines flagged as saturated yield reliable column densities.} 
\item[e] {\scriptsize Energy to attain ionization state of Ion 1} 
\item[f] {\scriptsize Energy to attain ionization state of Ion 2} 
\end{tablenotes} 
\end{threeparttable} 
\end{center} 
\label{table:ionioncorr} 
\end{table*} 


==> EWCDtable.tex <==
\begin{table}[!t] 
\caption{Limiting equivalent widths and path lengths calculated as functions of column density.} 
\begin{center} 
\begin{threeparttable} 
\begin{tabular}{ccccc} 
\toprule 
log N(C~\textsc{iv}) [cm$^{-2}$] & W$_{\rm 1550}$\tnote{a} \ [m\AA] & \Dz  & \DX  & \dNdz\tnote{b} \\ 
\hline 
13.0 & 19 & 0.1 & 0.1 & - \\[4pt]  
13.1 & 24 & 0.5 & 0.5 & - \\[4pt]  
13.2 & 29 & 0.8 & 0.8 & - \\[4pt]  
13.3 & 35 & 1.1 & 1.3 & 7.80$^{+2.4}_{-1.4}$ \\[4pt]  
13.4 & 43 & 1.7 & 1.9 & 6.79$^{+2.1}_{-1.2}$ \\[4pt]  
13.5 & 54 & 1.8 & 2.0 & 6.79$^{+2.1}_{-1.2}$ \\[4pt]  
13.6 & 67 & 2.8 & 3.1 & 5.51$^{+1.6}_{-1.0}$ \\[4pt]  
13.7 & 83 & 4.0 & 4.4 & 4.59$^{+1.4}_{-0.8}$ \\[4pt]  
13.8 & 102 & 4.3 & 4.7 & 3.22$^{+1.1}_{-0.6}$ \\[4pt]  
13.9 & 124 & 5.5 & 6.1 & 2.59$^{+0.9}_{-0.5}$ \\[4pt]  
14.0 & 150 & 7.1 & 7.9 & 2.43$^{+0.8}_{-0.5}$ \\[4pt]  
14.1 & 178 & 8.7 & 9.6 & 1.56$^{+0.7}_{-0.4}$ \\[4pt]  
14.2 & 208 & 9.9 & 11.1 & 0.91$^{+0.6}_{-0.3}$ \\[4pt]  
14.3 & 241 & 10.9 & 12.1 & 0.52$^{+0.5}_{-0.2}$ \\[4pt]  
14.4 & 275 & 11.6 & 12.9 & 0.17$^{+0.4}_{-0.1}$ \\[4pt]  
14.5 & 310 & 12.0 & 13.4 & 0.08$^{+0.3}_{-0.1}$ \\[4pt]  
14.6 & 345 & 12.3 & 13.8 & 0.08$^{+0.3}_{-0.1}$ \\[4pt]  
14.7 & 379 & 12.5 & 14.0 & - \\[4pt]  
14.8 & 412 & 12.7 & 14.2 & - \\[4pt]  
14.9 & 442 & 12.8 & 14.3 & - \\[4pt]  
15.0 & 468 & 12.9 & 14.4 & - \\ 
\hline 
\end{tabular} 
\begin{tablenotes} 
\item[a]{\scriptsize Equivalent width corresponding to \cfourcol\ in Column 1} 
\item[b]{\scriptsize Cumulative number of detected absorbers per redshift path length (see Eq. \ref{eq:dndz})} 
\end{tablenotes} 
\end{threeparttable} 
\end{center} 
\label{tab:EWCD} 
\end{table}


==> QSOinfo.tex <==
\begin{longtable}{lrrc} 
\tabletypesize{\scriptsize} 
\tablewidth{0pt} 
\tablecaption{QSO Sample for \cfour\ survey.} 
\tablehead{\colhead{QSO Name}  & \colhead{$\alpha$ (J2000)} & \colhead{$\delta$ (J2000)} & \colhead{$z_{\rm qso}$} \\ \ & \multicolumn{2}{c}{(degrees)} & \ }
SDSS J001224.01-102226.5 & 3.1001 & $-10.3740$ & 0.228 \\ 
SDSS J004222.29-103743.8 & 10.5929 & $-10.6288$ & 0.424 \\ 
SDSS J015530.02-085704.0 & 28.8751 & $-8.9511$ & 0.165 \\ 
SDSS J021218.32-073719.8 & 33.0764 & $-7.6222$ & 0.174 \\ 
SDSS J022614.46+001529.7 & 36.5603 & $0.2583$ & 0.615 \\ 
PHL 1337 & 38.7808 & $-4.0349$ & 1.437 \\ 
SDSS J024250.85-075914.2 & 40.7119 & $-7.9873$ & 0.377 \\ 
SDSS J025937.46+003736.3 & 44.9061 & $0.6268$ & 0.534 \\ 
SDSS J031027.82-004950.7 & 47.6159 & $-0.8308$ & 0.080 \\ 
SDSS J040148.98-054056.5 & 60.4541 & $-5.6824$ & 0.570 \\ 
FBQS 0751+2919 & 117.8013 & $29.3273$ & 0.915 \\ 
SDSS J080359.23+433258.4 & 120.9968 & $43.5496$ & 0.449 \\ 
SDSS J080908.13+461925.6 & 122.2839 & $46.3238$ & 0.657 \\ 
SDSS J082024.21+233450.4 & 125.1009 & $23.5807$ & 0.470 \\ 
SDSS J082633.51+074248.3 & 126.6396 & $7.7134$ & 0.311 \\ 
SDSS J084349.49+411741.6 & 130.9562 & $41.2949$ & 0.990 \\ 
SDSS J091029.75+101413.6 & 137.6240 & $10.2371$ & 0.463 \\ 
SDSS J091235.42+295725.4 & 138.1476 & $29.9571$ & 0.305 \\ 
SDSS J091440.38+282330.6 & 138.6683 & $28.3918$ & 0.735 \\ 
SDSS J092554.43+453544.4 & 141.4768 & $45.5957$ & 0.329 \\ 
SDSS J092554.70+400414.1 & 141.4779 & $40.0706$ & 0.471 \\ 
SDSS J092837.98+602521.0 & 142.1583 & $60.4225$ & 0.296 \\ 
SDSS J092909.79+464424.0 & 142.2908 & $46.7400$ & 0.240 \\ 
SDSS J093518.19+020415.5 & 143.8258 & $2.0710$ & 0.649 \\ 
SDSS J094331.61+053131.4 & 145.8817 & $5.5254$ & 0.564 \\ 
SDSS J094621.26+471131.3 & 146.5886 & $47.1920$ & 0.230 \\ 
SDSS J094733.21+100508.7 & 146.8884 & $10.0858$ & 0.139 \\ 
SDSS J094952.91+390203.9 & 147.4705 & $39.0344$ & 0.365 \\ 
SDSS J095000.73+483129.3 & 147.5031 & $48.5248$ & 0.589 \\ 
SDSS J095915.65+050355.1 & 149.8152 & $5.0653$ & 0.162 \\ 
SDSS J100102.55+594414.3 & 150.2606 & $59.7373$ & 0.746 \\ 
SDSS J100902.06+071343.8 & 152.2586 & $7.2289$ & 0.456 \\ 
SDSS J101622.60+470643.3 & 154.0942 & $47.1120$ & 0.822 \\ 
SDSS J102218.99+013218.8 & 155.5791 & $1.5386$ & 0.789 \\ 
PG1049-005 & 162.9643 & $-0.8549$ & 0.359 \\ 
SDSS J105945.23+144142.9 & 164.9385 & $14.6953$ & 0.631 \\ 
SDSS J105958.82+251708.8 & 164.9951 & $25.2858$ & 0.662 \\ 
SDSS J110312.93+414154.9 & 165.8039 & $41.6986$ & 0.402 \\ 
SDSS J110406.94+314111.4 & 166.0289 & $31.6865$ & 0.434 \\ 
SDSS J111239.11+353928.2 & 168.1630 & $35.6578$ & 0.636 \\ 
SDSS J111754.31+263416.6 & 169.4763 & $26.5713$ & 0.421 \\ 
SDSS J112114.22+032546.7 & 170.3092 & $3.4297$ & 0.152 \\ 
SDSS J112244.89+575543.0 & 170.6870 & $57.9286$ & 0.906 \\ 
SDSS J113327.78+032719.1 & 173.3658 & $3.4553$ & 0.525 \\ 
SDSS J113457.62+255527.9 & 173.7401 & $25.9244$ & 0.710 \\ 
PG1148+549 & 177.8353 & $54.6259$ & 0.975 \\ 
SDSS J115758.72-002220.8 & 179.4947 & $-0.3725$ & 0.260 \\ 
PG1202+281 & 181.1754 & $27.9033$ & 0.165 \\ 
SDSS J120720.99+262429.1 & 181.8375 & $26.4081$ & 0.324 \\ 
PG1206+459 & 182.2417 & $45.6765$ & 1.163 \\ 
SDSS J121037.56+315706.0 & 182.6565 & $31.9517$ & 0.389 \\ 
SDSS J121114.56+365739.5 & 182.8107 & $36.9610$ & 0.171 \\ 
SDSS J122035.10+385316.4 & 185.1463 & $38.8879$ & 0.376 \\ 
SDSS J123304.05-003134.1 & 188.2669 & $-0.5262$ & 0.471 \\ 
SDSS J123335.07+475800.4 & 188.3962 & $47.9668$ & 0.382 \\ 
SDSS J123604.02+264135.9 & 189.0168 & $26.6933$ & 0.209 \\ 
SDSS J124154.02+572107.3 & 190.4751 & $57.3520$ & 0.583 \\ 
SDSS J124511.25+335610.1 & 191.2969 & $33.9361$ & 0.711 \\ 
SDSS J132222.68+464535.2 & 200.5945 & $46.7598$ & 0.375 \\ 
SDSS J132704.13+443505.0 & 201.7672 & $44.5847$ & 0.331 \\ 
SDSS J133045.15+281321.4 & 202.6881 & $28.2226$ & 0.417 \\ 
SDSS J133053.27+311930.5 & 202.7220 & $31.3252$ & 0.242 \\ 
PG1338+416 & 205.2533 & $41.3872$ & 1.214 \\ 
SDSS J134206.56+050523.8 & 205.5274 & $5.0900$ & 0.266 \\ 
SDSS J134231.22+382903.4 & 205.6301 & $38.4843$ & 0.172 \\ 
SDSS J134246.89+184443.6 & 205.6954 & $18.7455$ & 0.383 \\ 
SDSS J134251.60-005345.3 & 205.7150 & $-0.8959$ & 0.326 \\ 
SDSS J135625.55+251523.7 & 209.1065 & $25.2566$ & 0.164 \\ 
SDSS J135712.61+170444.1 & 209.3026 & $17.0789$ & 0.150 \\ 
PG1407+265 & 212.3496 & $26.3059$ & 0.940 \\ 
SDSS J141910.20+420746.9 & 214.7925 & $42.1297$ & 0.873 \\ 
SDSS J143511.53+360437.2 & 218.7980 & $36.0770$ & 0.429 \\ 
SDSS J143726.14+504555.8 & 219.3589 & $50.7655$ & 0.783 \\ 
LBQS 1435-0134 & 219.4512 & $-1.7863$ & 1.308 \\ 
SDSS J144511.28+342825.4 & 221.2970 & $34.4737$ & 0.697 \\ 
SDSS J145108.76+270926.9 & 222.7865 & $27.1575$ & 0.064 \\ 
SDSS J151428.64+361957.9 & 228.6194 & $36.3328$ & 0.695 \\ 
SDSS J152139.66+033729.2 & 230.4153 & $3.6248$ & 0.126 \\ 
PG1522+101 & 231.1022 & $9.9748$ & 1.328 \\ 
SDSS J154553.48+093620.5 & 236.4729 & $9.6057$ & 0.665 \\ 
SDSS J155048.29+400144.9 & 237.7012 & $40.0291$ & 0.497 \\ 
SDSS J155304.92+354828.6 & 238.2705 & $35.8079$ & 0.722 \\ 
SDSS J155504.39+362848.0 & 238.7683 & $36.4800$ & 0.714 \\ 
SDSS J161649.42+415416.3 & 244.2059 & $41.9046$ & 0.440 \\ 
SDSS J161711.42+063833.4 & 244.2976 & $6.6426$ & 0.229 \\ 
SDSS J161916.54+334238.4 & 244.8189 & $33.7107$ & 0.471 \\ 
PG1630+377 & 248.0047 & $37.6306$ & 1.476 \\ 
SDSS J225738.20+134045.4 & 344.4092 & $13.6793$ & 0.594 \\ 
SDSS J234500.43-005936.0 & 356.2518 & $-0.9933$ & 0.789 \\ 
\label{tab:QSOinfo} 
\end{longtable} 


==> StackLatexSnippets.tex <==
\begin{figure*}[!b] 
\centering 
\includegraphics[width=0.9\textwidth,height=0.9\textheight,keepaspectratio]{{stacktile_1}.pdf} 
\caption{Spectra and fitted Voigt profiles for our \cfour~absorber sample.  For each system, at least one transition is shown for every ion detected, and each component is colored to match components of other species approximately aligned in velocity.  Profiles of interloping lines from other systems that were included in a fit are marked with purple x's, while the overalll fit is shown in maroon.  The error vector is plotted in light red.} 
\end{figure*} 

\setcounter{figure}{\value{figure}-1} 
\begin{figure*}[!h] 
\centering 
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{{stacktile_2}.pdf} 
\caption{continued.} 
\end{figure*} 

\setcounter{figure}{\value{figure}-1} 
\begin{figure*}[!h] 
\centering 
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{{stacktile_3}.pdf} 
\caption{continued.} 
\end{figure*} 

\setcounter{figure}{\value{figure}-1} 
\begin{figure*}[!h] 
\centering 
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{{stacktile_4}.pdf} 
\caption{continued.} 
\end{figure*} 

\setcounter{figure}{\value{figure}-1} 
\begin{figure*}[!h] 
\centering 
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{{stacktile_5}.pdf} 
\caption{continued.} 
\end{figure*} 

\setcounter{figure}{\value{figure}-1} 
\begin{figure*}[!h] 
\centering 
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{{stacktile_6}.pdf} 
\caption{continued.} 
\end{figure*} 

\setcounter{figure}{\value{figure}-1} 
\begin{figure*}[!h] 
\centering 
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{{stacktile_7}.pdf} 
\caption{continued.} 
\end{figure*} 

\setcounter{figure}{\value{figure}-1} 
\begin{figure*}[!h] 
\centering 
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{{stacktile_8}.pdf} 
\caption{continued.} 
\end{figure*} 

\setcounter{figure}{\value{figure}-1} 
\begin{figure*}[!h] 
\centering 
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{{stacktile_9}.pdf} 
\caption{continued.} 
\end{figure*} 

\setcounter{figure}{\value{figure}-1} 
\begin{figure*}[!h] 
\centering 
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{{stacktile_10}.pdf} 
\caption{continued.} 
\end{figure*} 

\setcounter{figure}{\value{figure}-1} 
\begin{figure*}[!h] 
\centering 
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{{stacktile_11}.pdf} 
\caption{continued.} 
\end{figure*} 


